A DECam Search for Explosive Optical Transients Associated with IceCube Neutrinos

In this work, we investigate the likelihood of association between realtime, TeV-PeV energy neutrino alerts from IceCube and optical counterparts in the form of core-collapse supernovae (CC SNe). The optical follow-up of IceCube alerts requires two main instrumental capabilities: (1) deep imaging, since 73\% of neutrinos would come from CC SNe at redshifts $z > 0.3$, and (2) a large field of view (FoV), since typical IceCube muon neutrino pointing accuracy is on the order of $\sim1$~deg. With Blanco/DECam ($gri$ to 24th magnitude and $2.2$~deg diameter FoV), we performed a triggered optical follow-up observation of two IceCube alerts, IC170922A and IC171106A on $\sim6$~nights during the $\sim3$~weeks following each alert. For the IC170922A (IC171106A) follow-up observations, we expect that 12.1\% (9.5\%) of coincident CC SNe at $z \lesssim 0.3$ are detectable, and that on average, 0.23 (0.07) unassociated SNe in the neutrino 90\% containment regions also pass our selection criteria. We find two candidate CC SNe that are temporally coincident with the neutrino alerts in the FoV, but none in the 90\% containment regions, which is statistically consistent with expected rates of background CC SNe for these observations. If CC SNe are the dominant source of TeV-PeV neutrinos, we would expect an excess of coincident CC SNe to be detectable at the $3\sigma$ confidence level using DECam observations similar to those of this work for $\sim60$ ($\sim200$) neutrino alerts with (without) redshift information for all candidates.

==> authors.tex <==
\correspondingauthor{Robert Morgan}
\email{robert.morgan@wisc.edu}

\author[]{Robert Morgan}
\affil{University of Wisconsin-Madison}
\affil{Large Synoptic Survey Telescope Corporation Data Science Fellowship Program}

\author[]{Keith Bechtol}
\affil{University of Wisconsin-Madison}
\affil{Large Synoptic Survey Telescope}


%R. Kessler, 
%M. Sako, 
%K. Herner, 
%Z. Doctor, 
%D. Scolnic, 
%I. Sevilla-Noarbe, 
%A. Franckowiak, 
%N. Neilson, 
%M. Kowalski, 
%B. Thomas, 
%E. Swann, 
%K. Vivas, 
%D. Brout, 
%F. Paz-Chinchon, 
%E. Neilson, 
%T. Diehl, 
%M. Soares-Santos


